Understanding In-Context Learning in Transformers and LLMs by Learning to Learn Discrete Functions

In order to understand the in-context learning phenomenon, recent works have adopted a stylized experimental framework and demonstrated that Transformers can learn gradient-based learning algorithms for various classes of real-valued functions. However, the limitations of Transformers in implementing learning algorithms, and their ability to learn other forms of algorithms are not well understood. Additionally, the degree to which these capabilities are confined to attention-based models is unclear. Furthermore, it remains to be seen whether the insights derived from these stylized settings can be extrapolated to pretrained Large Language Models (LLMs). In this work, we take a step towards answering these questions by demonstrating the following: (a) On a test-bed with a variety of Boolean function classes, we find that Transformers can nearly match the optimal learning algorithm for 'simpler' tasks, while their performance deteriorates on more 'complex' tasks. Additionally, we find that certain attention-free models perform (almost) identically to Transformers on a range of tasks. (b) When provided a teaching sequence, i.e. a set of examples that uniquely identifies a function in a class, we show that Transformers learn more sample-efficiently. Interestingly, our results show that Transformers can learn to implement two distinct algorithms to solve a single task, and can adaptively select the more sample-efficient algorithm depending on the sequence of in-context examples. (c) Lastly, we show that extant LLMs, e.g. LLaMA-2, GPT-4, can compete with nearest-neighbor baselines on prediction tasks that are guaranteed to not be in their training set.

==> sections/limitations.tex <==
\section{Limitations}\label{sec:Limitations}





% A general limitation of this line of work is that most of the results are primarily confined to artificial datasets. Although such formal languages provide us with a controlled setting and clarity regarding the precise nature of the problem, the relation to practical tasks remains unclear. Hence, while our results highlight the contrast in the performance between the two types of architectures, its precise implications on real-world tasks remain unclear.


% There are two negative results that do not support our hypothesis. (a) All the experiments discussed in the main paper are on strings of fixed lengths. We conducted some experiments on tasks with variable length sequences which in some sense have low sensitivity. The tasks can be seen as a variable length extension of sparse parities and sparse majorities. Unlike the fixed length setting, we found both LSTMs and Transformers perform similarly on those tasks. See Section \ref{app:varlen} in the Appendix for more details. (b) Although we found Transformers to consistently converge to low sensitivity functions in the case of Boolean functions, we did not find similar behaviour on sentiment classification datasets such as SST and IMDB.

% A caveat with empirical studies such as this is that the results depend on the hyperparameters and other aspects of the experimental setup. While we have tried to be as thorough as possible with hyperparameter tuning, there is always a chance that the results or behaviour could differ for some hyperparameter.


% \section*{Acknowledgments}

% We would like to thank Michael Hahn, Ard Louis, Kabir Ahuja, and our colleagues at the University of Oxford for helpful discussions and providing valuable feedback.



